Domain Adaptation by Topology Regularization

Deep learning has become the leading approach to assisted target recognition. While these methods typically require large amounts of labeled training data, domain adaptation (DA) or transfer learning (TL) enables these algorithms to transfer knowledge from a labelled (source) data set to an unlabelled but related (target) data set of interest. DA enables networks to overcome the distribution mismatch between the source and target that leads to poor generalization in the target domain. DA techniques align these distributions by minimizing a divergence measurement between source and target, making the transfer of knowledge from source to target possible. While these algorithms have advanced significantly in recent years, most do not explicitly leverage global data manifold structure in aligning the source and target. We propose to leverage global data structure by applying a topological data analysis (TDA) technique called persistent homology to TL. In this paper, we examine the use of persistent homology in a domain adversarial (DAd) convolutional neural network (CNN) architecture. The experiments show that aligning persistence alone is insufficient for transfer, but must be considered along with the lifetimes of the topological singularities. In addition, we found that longer lifetimes indicate robust discriminative features and more favorable structure in data. We found that existing divergence minimization based approaches to DA improve the topological structure, as indicated over a baseline without these regularization techniques. We hope these experiments highlight how topological structure can be leveraged to boost performance in TL tasks.

==> Content/__latexindent_temp.tex <==
\section{Introduction}
\label{sec:intro}  % \label{} allows 
\begin{figure}[ht]
  \begin{centering}
  $ \vcenter{\hbox{\begin{overpic}[unit=1mm, scale = .75]{Figs/introd5b4_1.pdf}
  \put(11, 10){\small{dim 1}}
  \put(17,60){\small{dim 2}}
  \put(55, 18){\small{dim 3}}
  \put(75,25){\huge{$\longrightarrow$}}
  \put(62,32){By matching topology}
  \end{overpic}}}$ 
  \hspace{3cm}
  $\vcenter{\hbox{\begin{overpic}[unit=1mm, scale = .75]{Figs/afterd7.pdf}
  \put(2, -3){\small{dim 1}}
  \put(18,50){\small{dim 2}}
  \put(61,9){\small{dim 3}}
  \end{overpic}}}$
    \end{centering}
        \caption{Manifolds represent global data structure. Here the grey disk with two holes represents the source data manifold, while the dark grey dots represent individual source image examples. The blue annulus represents the target data manifold, and the dark blue dots represent the target image examples. The left side image shows a possible outcome of feature extraction without topological considerations. The right side shows the theoretical outcome with topology  regularization.}
        \label{introfigure}
    \end{figure}

Recent advances in the field of machine learning have focused largely on deep neural networks. These networks learn feature representations that can be used in a variety of applications including object recognition, natural language processing, and scene segmentation from sensor data.  Unfortunately, deep neural networks need large quantities of labeled training data. Moreover, the data must be domain and task specific. For example, classifying images of vehicles requires training images taken during the day, night, and under a variety of weather conditions for the system to work reliably under those various conditions. Unfortunately this type of data can be expensive or impractical to obtain. This lack of labelled data could be resolved if deep neural networks could be trained on one data set, then \emph{transferred} to a different data set. Unfortunately, different dataset features may be distorted such that the probability distributions do not match, which leads to poor generalization \cite{Pan2010}. 

Mitigating the representation shift is a primary focus of \gls{DA} research. Previous attempts fine tune networks to the new data set \cite{Yos}. This approach assumes the source and target feature spaces are similar and does not accommodate for the large differences in data distributions that can come from different sensor types. \gls{DA} attempts to overcome this by aligning the feature representation of a labeled data set - called the source data - with that of an unlabeled data set - called the target data. Past attempts have aligning the distributions by minimizing a measure of divergence  - such as by maximum mean discrepency \cite{Long2017, Long2018}, Kullbach-Leibler divergence\cite{Kullback51}, or a domain loss\cite{ADDA}. Some of these measures emphasize the local interactions between points. By contrast, a topological regularization would use the global structure of the source and target data manifolds  to align them in the common latent space.

In this paper we investigate using persistent homology, a tool from \gls{TDA}, to analyze and align the global structure of the source and target feature representations of a \gls{NN}. The idea is illustrated in Fig.~\ref{introfigure} for source and target datasets. This method first constructs a manifold from a point cloud by connecting data points that are within some variable threshold distance. Persistent homology defines a persistence diagram by summarizing the number and size (lifetimes) of holes and voids (topological singularities) in the data manifold formed by the point cloud. These persistence diagrams summarize the topological structure, and can be used to regularize the network's feature representation.

Our empirical findings are summarized as follows: We examined what features persistent homology can detect in data samples. We found that longer lifetimes indicate favorable features and structure in the data manifold. We then analyzed what impact current state of the art techniques have on the global structure of feature representations and where in the network architecture this structure can be useful. Existing divergence minimization based approaches to \gls{DA} improved the topological structure, as indicated by longer lifetimes over a baseline network. Also, we found that as data goes through layers of \gls{CNN}, there is an increase in topological structure after passing through the second convolutional layer. This increase is later broken down toward the discriminative parts of the network architecture. Guided by the results of these experiments, we designed a network that forces the global structure of the source and target feature representations to be topologically similar by minimizing the Wasserstein distance between their persistence diagrams in the latent network layers. We found no transfer improvement beyond the existing \gls{DA} approaches, and discuss possibilties for this finding. Taken collectively, our experiments show that persistent homology is useful for identifying robust representations in general, but may be less useful for divergence minimization.

The paper is organized as follows: We provide the technical background in Sec.~\ref{sec:Background} before reviewing related work and the methodology in Sections~\ref{sec:related} and \ref{sec:methods}, respectively. The experiments and analysis of Sec.~\ref{sec:experiments} provide the bulk of our reserach contribution. Finally, we close with a discussion and conclusion.
